NTIRE 2025 Challenge on Day and Night Raindrop Removal for Dual-Focused Images: Methods and Results

This paper reviews the NTIRE 2025 Challenge on Day and Night Raindrop Removal for Dual-Focused Images. This challenge received a wide range of impressive solutions, which are developed and evaluated using our collected real-world Raindrop Clarity dataset. Unlike existing deraining datasets, our Raindrop Clarity dataset is more diverse and challenging in degradation types and contents, which includes day raindrop-focused, day background-focused, night raindrop-focused, and night background-focused degradations. This dataset is divided into three subsets for competition: 14,139 images for training, 240 images for validation, and 731 images for testing. The primary objective of this challenge is to establish a new and powerful benchmark for the task of removing raindrops under varying lighting and focus conditions. There are a total of 361 participants in the competition, and 32 teams submitting valid solutions and fact sheets for the final testing phase. These submissions achieved state-of-the-art (SOTA) performance on the Raindrop Clarity dataset. The project can be found at https://lixinustc.github.io/CVPR-NTIRE2025-RainDrop-Competition.github.io/.

==> sec/4_Teams_and_Methods.tex <==
% \clearpage
% \setcounter{page}{1}
% \maketitlesupplementary


\section{Teams and Methods}
\label{sec:teams_and_methods}
Please find the details of all \textbf{32 teams and their methods} in the \textbf{Supplementary}.
\subsection{Miracle}
% revised by Miracle, please finish it before 12/04/2025.
\begin{figure}[htbp]
    \centering
    \includegraphics[width=1.0\linewidth]{figs/Miracle_1.png}
    \caption{The framework of STRRNet\yeying{, proposed by Team Miracle}}
    \label{fig:Miracle_1}
\end{figure}


\begin{figure}[htbp]
    \centering
    \includegraphics[width=1.0\linewidth]{figs/Miracle_3.png}
    \caption{Semantic Guidance Module \yeying{of STRRNet, proposed by Team Miracle}}
    \label{fig:Miracle_3}
\end{figure}

\begin{figure}[htbp]
    \centering
    \includegraphics[width=1.0\linewidth]{figs/Miracle_2.png}
    \caption{Training Strategy \yeying{of STRRNet}, proposed by Team Miracle}
    \label{fig:Miracle_2}
\end{figure}

This team proposes the STRRNet~\cite{rong2025STRRNet}, which is developed based on Restormer \cite{zamir2022restormer}\yeying{, as shown in Fig~\ref{fig:Miracle_1}.} They categorize the training images into four classes based on lighting conditions and raindrop types: night\_bg\_focus, night\_raindrop\_focus,
day\_bg\_focus, and day\_raindrop\_focus. \yeying{As shown in Fig~\ref{fig:Miracle_3}, a} text embedder is first trained on the labeled training set using these four categories. Then, they design a semantic
guidance module, which is added at the end of the Restormer encoder.
This module utilizes the encoded image features from Restormer to guide the decoder in performing distinct image restoration operations for the
four different types of images. Additionally, they introduce a background restoration
subnetwork at the output of Restormer, which consists of multiple
convolutional layers to enhance image details. 
The training strategy of STRRNet is illustrated in the Fig \ref{fig:Miracle_2}.
First, they train a pre-trained model on the original training dataset. This model is then used to perform inference on all frames within the same scene in the test set. The inferred images may still contain residual raindrops and artifacts. Since the background remains consistent across different time frames while raindrop positions vary temporally, this motivates them to perform median fusion across multiple frames from the same scene to obtain a median-fused image. Due to the dynamic nature of raindrop artifacts, their inconsistent locations across frames typically prevent them from appearing in the median values, whereas the stable background information is preserved. They then treat the median-fused image as a pseudo ground truth and use it in a semi-supervised fine-tuning phase to enhance the model’s raindrop removal capability on unlabeled images.
\\
\textbf{Training description}
The Adam optimizer is used for training, with a total of 500,000 iterations.
The learning rate is set to 0.0003 for the first 9,2000 iterations and then
gradually decays from 0.0003 to 0.000001 for the remaining iterations. Images
are randomly cropped to a fixed size of 128×128 for network training,
and geometric image augmentation is applied. The network is optimized
using the L1 loss function and the multi-scale SSIM loss function, with
weights of 1 and 0.2, respectively. All their experiments were conducted on
an RTX 4090.\\
\textbf{Testing description}
Use a sliding window to move across the image, applying the model for
rain removal on each window. Set the sliding window size to 128×128
with an overlap of 32. Then, obtain a median image by applying median
fusion to the images of the same scene. Finally, perform a weighted sum
of the median image and the original image to obtain the final output.\\





% This team proposed the method based on Restormer~\cite{zamir2022restormer}. They categorize images in the training set into four classes: night\_bg\_focus, night\_raindrop\_focus,
% day\_bg\_focus, and day\_raindrop\_focus. A text embedder is trained on the training set using these four categories. Then, they design a semantic guidance module, which is added at the end of the Restormer encoder. This module utilizes the encoded image features from Restormer to guide the decoder in performing distinct image restoration operations for the
% four different types of images. Additionally, they introduce a background restoration sub-network at the output of Restormer, which consists of multiple convolutional layers to enhance image details. The aforementioned model
% structure is trained on the training set to obtain a more robust model.



\subsection{EntroVision}
\begin{figure}[htbp]
\centering
\includegraphics[width=1.0\linewidth]{figs/EntroVision.png}
\caption{Overview of the technique \yeying{proposed by Team EntroVision} for raindrop removal.}
\label{fig:EntroVision}
\end{figure}

This team utilizes a two-stage approach to achieve raindrop removal in this challenge. The technical overview is shown in the Fig.~\ref{fig:EntroVision}. Given the impact of multi-scale features in image deraining~\cite{chen2024bidirectional,chen2023towards}, they pre-train the deraining model in the first stage using MSDT~\cite{chen2024rethinkingMSDT} on the RainDrop Clarity~\cite{jin2024raindrop} training set. To enhance the model's generalization capability, additional pre-training is conducted on the UAV-Rain1k~\cite{chang2024uavrain1k} dataset. Then, the pre-trained deraining model is utilized to obtain the pseudo-ground-truth images for testing images for the test-time learning of the second stage.

% \begin{figure}
%     \centering
%     \includegraphics[width=1.0\linewidth]{figs_revise/EntroVision-training.png}
%     \caption{Overview of the technique for raindrop removal.}
%     \label{fig:EntroVision-training}
% \end{figure}

In the second stage of the process, they performed fine-tuning using the test samples and the generated paired pseudo ground-truth images. This approach provides a clear direction for transferring pretrained knowledge, rather than simply relying on the model's generalization ability. Subsequently, they process the testing inputs using this fine-tuned deraining model to obtain the final output results. Notably, they designed the deraining network specifically according to the characteristics of the dataset used. To address scenarios where blurry and clear backgrounds might coexist, they employ median filtering to preserve edge information and avoid excessive blurring. Through the above two-stage processing strategies and the specially designed median
filtering technique, they obtain clear deraining results. 

%The three-stage training details are shown in Fig.~\ref{fig:EntroVision-training}.

% \noindent\textbf{Training Details}
% They pre-train the model using the RainDrop Clarity~\cite{jin2024raindropclarity} training dataset. To enhance the model’s generalization ability, they additionally introduce the UAV-Rain1k\cite{chang2024uavrain1k} dataset during the pretraining phase. They then process the test set using the pretrained weights to generate paired pseudo GT. Next, they fine-tune the model using the test set and pseudo-GT to generate the final weights.

% \noindent\textbf{Testing Details}
% In the testing phase, they process the test inputs using the fine-tuned weights and then further refine the restoration results using the designed median filtering module.



\subsection{IIRLab}
\begin{figure}[htbp]
    \centering
    \includegraphics[width=1.0\linewidth]{figs_revise/IIRLab.png}
    \caption{\yeying{The pipeline of the method proposed by Team IIRLab}}
    \label{fig:IIRLab}
\end{figure}

This team observed that the raindrop dataset used in this challenge differs significantly from existing raindrop removal datasets. Traditional datasets primarily focus on background clarity during image shooting, resulting in clean backgrounds and blurry raindrops in the foreground. In such cases, simply removing the raindrops is sufficient to recover a clear background. However, the dataset in this challenge includes a notable portion of images where the camera is focused on the raindrops during shooting, leading to clean raindrops and blurred backgrounds. This introduces a new challenge: removing not only the raindrops themselves but also mitigating background blur caused by defocus, to ultimately recover a clean draining image.

% The raindrop dataset used this time has some images that are focused on the foreground raindrops during shooting, which can result in clear raindrops and blurry backgrounds. This poses a new challenge to the problem of removing raindrops, not only from the foreground but also from the background blur caused by defocusing, in order to ultimately restore a clear background.

Based on this new question, this team has chosen the Histoformer~\cite{sun2024restoringhistogram} network as their raindrop removal model\yeying{, as shown in Fig~\ref{fig:IIRLab}}. Histoformer is a transformer-based model designed to restore images degraded by severe weather conditions. It incorporates a histogram self-attention mechanism, which sorts and segments spatial features into intensity-based bins and applies self-attention within each bin. This enables the model to focus on spatial features across dynamic intensity ranges and handle long-range dependencies between similarly degraded pixels. Built upon Restormer~\cite{zamir2022restormer}, Histoformer is well-suited for addressing both raindrop artifacts and defocus blur, making it a strong candidate for this task. Based on its architecture and prior performance, the team chose Histoformer as the core model for this challenge.



% Histoformer proposes an effective histogram converter (Histoformer) for restoring images affected by severe weather conditions. Histoformer is a transformer-based model for restoring severe weather images, capable of restoring clear images in various adverse weather conditions. It is supported by a mechanism called histogram self-attention, which sorts and segments spatial features into intensity-based bins. Then, it applies self-attention to the bin or each bin to selectively focus on spatial features of the dynamic range and process similar degraded pixels at long distances together.

% Histoformer is developed based on Restormer~\cite{zamir2022restormer}, so they believe that it can not only complete the task of removing raindrops but also the task of removing defocused blur. Therefore, they ultimately chose to use the Histoformer network to complete the competition task.


\noindent\textbf{Training Details.}
This team utilized all image pairs provided in the training set, consisting of raindrop-degraded images (Drop) and their corresponding clean background images (Clean). From this, they extracted 1,200 image pairs for validation, including 400 daytime and 800 nighttime samples. For training, they employed a two-stage training strategy that combines regular training with subsequent fine-tuning. In the first stage, the draining model was trained for 300,000 iterations using the default Histoformer configuration. In the second stage, the model was fine-tuned for an additional 13,000 iterations using only the $\mathcal{L}_1$ loss function. This progressive training approach effectively enhanced model performance, leading to improved final results.

\noindent\textbf{Implememtation Details.}
The implementation is based on PyTorch and was conducted on an NVIDIA RTX 3090 GPU. The network was trained for a total of 300,000 iterations, with an initial batch size of 6 and a patch size of $128\times 128$, following a progressive learning strategy. The team employed the AdamW optimizer with an initial learning rate of $3 \times 10^{-4}$ for the first 92,000 iterations, which was then gradually reduced to $1 \times 10^{-6}$ using a cosine annealing schedule over the remaining 208,000 iterations.
The number of blocks at each stage was set as $L_{i \in {1,2,3,4}} = {4, 4, 6, 8}$, and the channel dimension was fixed at $C = 36$. The channel expansion factor in the DGFF module was set to $r = 2.667$. The number of self-attention heads at each stage was configured as ${1, 2, 4, 8}$, respectively. For data augmentation, horizontal and vertical flips were applied randomly during training.


\subsection{PolyRain}
\begin{figure}[htbp]
    \centering
    \includegraphics[width=1.0\linewidth]{figs_revise/PolyRain.png}
    \caption{\yeying{The pipeline of the method proposed by Team PolyRain}}
    \label{fig:PolyRain}
\end{figure}

This team initialized and trained a dense X-Restormer model with the given dataset based on Restormer~\cite{zamir2022restormer}. After the first training stage, they finetuned the model on a larger patch size with different loss functions. The whole framework of this team is shown in Fig.~\ref{fig:PolyRain}.

\noindent\textbf{Training Details.}
The training process consists of two phases. In the first phase, the patch size of the training image is set to 256, with a batch size of 8, and a total of 3$\times$105 training iterations. The learning rate is set to $3e^{-4}$ and $\mathcal{L}_1$ Loss is used as the loss function. In the second phase, the model is fine-tuned with a $5e^{-5}$ learning rate and the image patch with 448 $\times$ 448. During this phase, the model is trained simultaneously using $\mathcal{L}_2$ Loss, LPIPS Loss, and SSIM Loss with weights of 1, 0.1, and 0.1, respectively, for 5$\times$104 iterations.

\noindent\textbf{Testing Details.}
To enhance the robustness of the model, the self-ensemble technique is employed. The implementation references the BasicSR library~\footnote{https://github.com/XPixelGroup/BasicSR}. 

\noindent\textbf{Implementation Details.}
This method is implemented based on the famous BasicSR framework~\cite{chan2021basicvsr,chen2024comparative} written in Python. They utilized the AdamW optimizer with an initial learning rate of $3e^{-4}$. Eight A100 GPUs were used for the model training, lasting for about 72 hours for 300000 iterations. In addition, the CosineAnnealingRestart-CyclicLR scheduler was chosen to restart the learning rate at a setting of $[92000, 208000]$. They did not use any efficient optimization strategy or extra datasets.



\subsection{H3FC2Z}
\begin{figure}[htbp]
    \centering
    \includegraphics[width=1.0\linewidth]{figs_revise/H3FC2Z.pdf}
    \caption{Dual kmeans fusion for RainDrop task \yeying{proposed by Team H3FC2Z}.}
    \label{fig:H3FC2Z}
\end{figure}
This team utilizes the RDDM~\cite{liu2024residualRDDM} as the deraining backbone and trained it with a patch size of $256\times 256$. Subsequently, the self-ensemble strategy used in the EDSR~\cite{lim2017enhancededsr} was improved by replacing the average ensemble with their ``Dual
Kmeans fusion" in the Fig.~\ref{fig:H3FC2Z}. Experimental results indicate that employing ``Dual Kmeans fusion"~\cite{chen2024ntirekmeans} increases the score of the RDDM baseline from 31.72 to 32.56. 

\noindent \textbf{Dual Kmeans Fusion.} 
Given a clean image $\mathcal{I}_{gt}$, several raindrop and blur degradations are added to $\mathcal{I}_{gt}$, obtaining $m$ images $(\mathcal{I}_{1}, \mathcal{I}_{2}, \cdots, \mathcal{I}_{m})$. As shown in Fig.~\ref{fig:H3FC2Z}, taking $\mathcal{I}_{1}$ as an example, they serve flipping and rotating as augmentations, generating $n$ images $(I_{1}, I_{2}, \cdots I_{n})$. \textbf{Stage-1}: The baseline model processes these images and obtains preliminary results $r_i = \text{Baseline}(I_i)$, where $i=1, 2, \cdots, n$. The images $r$ are flipped or rotated to a fixed angle and Kmeans fusion is performed to obtain $R_1$. \textbf{Stage-2}: After performing the above fusion on images $\mathcal{I}$, they get $m$ results $R_1, R_2, \cdots, R_m$. they perform Kmeans fusion on these $m$ results to get the final result image.


\noindent\textbf{Training and Testing Details.} The training dataset provided in this challenge is used for model training. To improve generalization, data augmentation techniques, including rotation and flipping are applied. The model is trained for 100,000 iterations using the AdamW optimizer with parameters $\beta_1 = 0.9$ and $\beta_2 = 0.95$, on a single NVIDIA A6000 GPU. Training is conducted with a batch size of 8, a learning rate of $3 \times 10^{-4}$, and a patch size of 256$\times$256. During inference, the authors adopt a Dual K-means fusion strategy to further enhance the model’s performance. Experimental results indicate that employing ``Dual Kmeans fusion" increases the score of RDDM~\cite{liu2024residualRDDM} baseline from 31.72 to 32.56. Specifically, Kmeans fusion in stage one increases the score of baseline from 31.72 to 32.26, and Kmeans fusion in stage two increases the score of baseline from 32.26 to 32.56.


% The training dataset provided in this challenge serves as training data. Employing rotating and flipping strategies enhances these images. Utilizing the AdamW optimizer ($\beta_1 = 0.9$, $\beta_2 = 0.95$), the authors conduct training for 100k iterations on 1 NVIDIA A6000 GPU, with a batch size of 8, a learning rate of $3\times e^{-4}$ and a patch size of 256 $\times$ 256. During inference, the authors implement the “Dual Kmeans fusion” strategy to enhance performance.

% \noindent\textbf{Testing Details}
% This team used the fusion strategy named Dual Kmeans fusion~\cite{chen2024ntirekmeans}. Given a clean image $\mathcal{I}_{gt}$, several raindrop and blur degradations are added to $\mathcal{I}_{gt}$, obtaining $m$ images ($\mathcal{I}_1, \mathcal{I}_2, \cdots , \mathcal{I}_m$). 
% As shown in Figure \ref{fig:H3FC2Z}, taking $\mathcal{I}_1$ as an example, they serve flipping and rotating as augmentations, generating $n$ images ($I_1, I_2, \cdots I_n$). 

% \textbf{Stage-1:} The baseline model then processes these images and obtains preliminary results $r_i = \text{Baseline}(I_i)$, where $i = 1, 2, \cdots , n$. The images $r$ are flipped or rotated to a fixed angle and Kmeans fusion is performed to obtain $R_1$. 

% \textbf{Stage-2:} After performing the above fusion on images $\mathcal{I}$, they get $m$ results $R_1, R_2, \cdots , R_m$. They perform kmeans fusion on these $m$ results to get the final result image.


\subsection{IIC Lab}
% \textcolor{red}{please add the references in your factsheet and figures in figs\_revise}

\begin{figure}[htbp]
    \centering
    \includegraphics[width=1.0\linewidth]{figs_revise/IICLab_v1.png}
    \caption{\yeying{The pipeline of the FA-Mamba proposed by Team IIC Lab}.}
    \label{fig:IICLab}
\end{figure}

This team developed an effective frequency-aware and Mamba-based network for image deraining, named FA-Mamba\yeying{, as shown in Fig.~\ref{fig:IICLab}}. Specifically, the key component of the proposed framework is the Wavelet Domain Restoration Module (WDRM) which contains a Dual-branch Feature Extraction Block (DFEB) that has superior local perception and global modeling capabilities and a Prior-Guided Module (PGM) that provides refined texture detail guidance for
feature extraction. It is worth mentioning that the refined texture details are obtained by enhancing the input high-frequency information through the High-Frequency Enhancement Module (HFEM).

\noindent\textbf{Training Details.}
During training, they utilized the Adam optimizer with a batch size of 1 and a patch size of 256 for a total of 80 iterations. The initial learning rate is fixed at $1e^{-4}$ for 60 iterations, and then decreased to $5e^{-5}$ for 20 iterations. No data augmentation techniques were applied. The entire framework is performed on PyTorch with an NVIDIA GeForce RTX 3090 GPU, which works in an end-to-end learning fashion without costly large-scale pertaining.


% BUPT CAT
\subsection{BUPT CAT}
\begin{figure}[htbp]
    \centering
    \includegraphics[width=1.0\linewidth]{figs_revise/BUPT_CAT.pdf}
    \caption{\yeying{The pipeline of the method proposed by Team BUPT CAT}.}
    \label{fig:BUPT_CAT}
\end{figure}

As shown in Fig.~\ref{fig:BUPT_CAT}, this team introduces a novel Consistent Patch Transformer (CPT) for dual-focused day and night raindrop removal task, which leverages a UNet-based architecture designed to enhance both spatial consistency and feature representation capability.
The framework comprises multiple Consistent Patch Transformer blocks, each consisting of two key components: Consistent Patch Self-Attention (CPSA) and a Feed-Forward Network (FFN). The model utilizes
the Test Time Local Converter (TLC) mechanism~\cite{chu2022improving} to effectively revisit global information aggregation and ensure robust and consistent feature learning with different patch sizes at training and testing.
The CPSA module is responsible for capturing both long-range dependencies and spatially consistent local details. Instead of using traditional window-based attention mechanisms, the CPSA module integrates a TLC-based feature aggregation and scaling strategy that maintains consistent patch sizes during training and testing, reducing spatial inconsistencies between training and testing. 

\noindent\textbf{Training Details.}
To reduce the training GPU memory, this team augments the input data by randomly cropping the input image into patches of the same size and performing strategies such as random rotation. 

\noindent\textbf{Testing Details.}
During the testing stage, in their self-attention part, they use the TLC strategy to segment and aggregate the full image into a series of patches of the same size as the training patch, and the rest of the model is the full image. This setup can effectively improve the inconsistency of the model’s patch size between training and testing, especially in the self-attention part.

\noindent\textbf{Implementation Details.}
This team utilizes the Pytorch framework with the NVIDIA GeForce RTX 4090. During training, they set the total batch size to 8, the initial learning rate from $5e^{-4}$ to $1e^{-5}$ with a scheduler in 500K iterations, and the patch size is set to 192$\times$192. For the loss function, they use $\mathcal{L}_1$loss and Fourier loss to constrain their model with weights of 1 and 0.1, respectively.
They train their framework using the Adam optimizer with $\beta1=0.9, \beta2=0.99$.
They set the number of channels to 64 in their network. The total training duration is approximately 80 hours. The training and test sets are official datasets provided by the dual-focused day and night raindrop removal challenge.

\subsection{WIRTeam}
\begin{figure}[htbp]
    \centering
    \includegraphics[width=0.95\linewidth]{figs_revise/WIRteam.png}
    \caption{\yeying{The pipeline of the method proposed by Team WIRteam}.}
    \label{fig:WIRTeam}
\end{figure}
Inspired by recent advancements~\cite{li2024promptcir,chen2023activating,potlapalli2023promptir,zamir2022restormer} in image restoration and image deraining, \yeying{this team} propose a novel multi-scale prompt-based image deraining approach (MPID) that incorporates both local and global attention mechanisms\yeying{, as shown in Fig.~\ref{fig:WIRTeam}.}
Specifically, given a degraded image $I \in R^{H \times W \times 3}$
, their model produces a corresponding clear image $\bar{I} \in R^ {H\times W \times 3}$ through a 4-level encoder-decoder framework. In the shadow two layers, they employ Residual Hybrid Attention Groups (RHAG)~\cite{chen2023activating} to capture detailed local features. For deeper layers, they integrate Transformer Blocks~\cite{zamir2022restormer} to facilitate cross-channel global feature extraction.
In the encoding phase, acknowledging the advantages of utilizing images at various resolutions for deraining tasks~\cite{chen2024bidirectional}, they additionally incorporate multi-scale image information (at 1/2 and 1/4 of the original resolution) to enhance auxiliary information during the encoding process. During decoding, considering the dual focus on raindrop-focus and background-focus images within the Raindrop Clarity dataset~\cite{ntire2025day}—which introduces both raindrop occlusions and background blurring—they introduce specialized
prompt mechanism~\cite{li2024promptcir}. These components are designed to address and decouple different types of degradation factors. Notably, Prompt Block, which integrates Prompt Generation Module (PGM) and Prompt Interaction Module (PIM), utilizes image-specific cues to effectively guide the image reconstruction process, thereby improving the clarity and quality of the restored images.\\
\noindent\textbf{Training Details.}
They employ the end-to-end training methodology, training their model for 400 epochs. The training procedure is based on the AdamW optimizer with the decay parameters $\beta_1 = 0.9$ and $\beta_2 = 0.99$. The initial learning rate is 2e-4 and gradually reduces to 1e-6 with the cosine annealing strategy. Horizontal and vertical flips are adopted for data augmentation. Furthermore, their training is merely based on the Raindrop Clarity dataset provided by the competition organizers, without the use of any extra datasets or pretrained models.\\
\noindent\textbf{Testing Details.}
During the testing phase, they preprocess the input images by padding them to the multiple of 32. This ensures that the dimensions of the input images are compatible with the architecture of their method. They don’t resort to any other means of Test-Time Augmentation during the testing phase.\\





\section*{Acknowledgments}
This work was partially supported by NSFC under Grant 623B2098 and the China Postdoctoral Science Foundation-Anhui Joint Support Program under Grant Number 2024T017AH. We thank the challenge sponsor: Eastern Institute for Advanced Study, Ningbo. This work was partially supported by the Humboldt Foundation. We thank the NTIRE 2025 sponsors: ByteDance, Meituan, Kuaishou, and University of Wurzburg (Computer Vision Lab).





